Hevelius Report: Visualizing Web-Based Mobility Test Data For Clinical Decision and Learning Support

Hevelius, a web-based computer mouse test, measures arm movement and has been shown to accurately evaluate severity for patients with Parkinson's disease and ataxias. A Hevelius session produces 32 numeric features, which may be hard to interpret, especially in time-constrained clinical settings. This work aims to support clinicians (and other stakeholders) in interpreting and connecting Hevelius features to clinical concepts. Through an iterative design process, we developed a visualization tool (Hevelius Report) that (1) abstracts six clinically relevant concepts from 32 features, (2) visualizes patient test results, and compares them to results from healthy controls and other patients, and (3) is an interactive app to meet the specific needs in different usage scenarios. Then, we conducted a preliminary user study through an online interview with three clinicians who were not involved in the project. They expressed interest in using Hevelius Report, especially for identifying subtle changes in their patients' mobility that are hard to capture with existing clinical tests. Future work will integrate the visualization tool into the current clinical workflow of a neurology team and conduct systematic evaluations of the tool's usefulness, usability, and effectiveness. Hevelius Report represents a promising solution for analyzing fine-motor test results and monitoring patients' conditions and progressions.

==> alt-text.tex <==
Figure 1: \Description{Figure of the interactive visualization tool \textit{Hevelius Report}. The figure contains four sub-figures. From left to right, the first sub-figure is a screenshot of the report's first page, where a set of summary plots are shown. The second sub-figure is a screenshot of the trajectory plots. The third sub-figure is a screenshot of the speed plots. The fourth sub-figure is a screenshot of additional information, including the loading plot of factor analysis, reading instructions, and other patient unique codes ordered by the number of \textit{Hevelius} sessions they have completed (in descending order). The interface is a single continuous page with a sidebar that allows users to jump to a particular section. The red asterisks (annotations in the figure; not present in the tool) indicate opportunities for user interactions.}
Figure 2: \Description{A loading plot in a heatmap format. The y axis is the list of 32 \textit{Hevelius} features, and the x-axis is the list of 6 factors. Each cell contains a numeric value that is the loading coefficient of the feature onto the factor. The higher the value, the darker the color (green) is.}
Figure 3: \Description{Example summary plot for a Parkinson's patient for a given timepoint and concept. There are two sub-plots in this image. On the left plot, the y-axis is distribution density, and the x-axis is the value of the chosen concept (a linear combination of the 32 features based on factor analysis). The value of the patient is plotted as a dotted verticle line (blue). The distributions of comparable healthy controls (in grey) and other patients (in blue) are plotted in the background. On the right plot, the y-axis is the concept value, and the x-axis is the days since the patient's first Hevelius session. The patient's values are plotted as a blue line, and the comparable healthy control averages are plotted as grey.}
Figure 4: \Description{Example trajectory plots for a Parkinson's patient. There are six sub-plots in this figure. Each column represents data from one Hevelius session. Each row represents data from a percentile (5th, 50th, or 95th) of the concept value. Within each sub-plot, a big orange circle on the right represents the target region of a Hevelius trial. The smaller blue dot on the left represents the starting point of the computer mouse. The dotted blue line represents the mouse's trajectory from the starting point to the target region. The grey dotted line represents a healthy control average trajectory.}
Figure 5: \Description{Example time-speed plots for a Parkinson's patient over two \textit{Hevelius} sessions. The plot contains six sub-plots. Each column represents data from one Hevelius session. Each row represents data from a percentile (5th, 50th, or 95th) of the concept value. Within each sub-plot, the y-axis measures speed, and the x-axis is the time point of a Hevelius trial. The speed profile of the mouse movement is presented as a line. The patient's line is blue, and the healthy control average is grey. The verticle dotted lines represent when the trial begins and when the patient starts to move the mouse.}
Figure 6: \Description{A dendrogram from hierarchical clustering. The x-axis is the Euclidean distance, and the y-axis is the list of 32 Hevelius features. The features are grouped based on their Euclidean distance.}
Figure 7: \Description{Comparison between an earlier version and a final version of the summary plots. The caption details the changes between the two versions.}
Figure 8: \Description{Comparison between two earlier versions and a final version of the trajectory plots. The caption details the changes between the three versions.}
Figure 9: \Description{Comparison between an earlier version and a final version of the speed plots. The caption details the changes between the two versions.}
Figure 10: \Description{A Figma frame of the first version of the user interface. It shows a one-page report with three panels. The top left panel contains the patient's basic information, such as age and gender. The bottom left panel contains the trajectory plots. The right panel contains the summary plots.}
